Characterization and Integration of the Singular Test Integrals in the Method-of-Moments Implementation of the Electric-Field Integral Equation

In this paper, we characterize the logarithmic singularities arising in the method of moments from the Green's function in integrals over the test domain, and we use two approaches for designing geometrically symmetric quadrature rules to integrate these singular integrands. These rules exhibit better convergence properties than quadrature rules for polynomials and, in general, lead to better accuracy with a lower number of quadrature points. We demonstrate their effectiveness for several examples encountered in both the scalar and vector potentials of the electric-field integral equation (singular, near-singular, and far interactions) as compared to the commonly employed polynomial scheme and the double Ma--Rokhlin--Wandzura (DMRW) rules, whose sample points are located asymmetrically within triangles.

==> packages.tex <==
%\usepackage[margin=1in]{geometry}
\usepackage{amsmath,amsfonts,mathtools,amssymb}
\usepackage[T1]{fontenc}%\usepackage{lmodern}
\usepackage{booktabs}
\makeatletter
\let\MYcaption\@makecaption
\makeatother



\makeatletter
\let\@makecaption\MYcaption
\makeatother
\usepackage{xcolor}
\usepackage{hyperref}
\hypersetup{hidelinks}
%\captionsetup*{font=normalsize,labelsep=quad}
\usepackage{multirow}
\usepackage{placeins}
\usepackage{etoolbox}
\usepackage{dblfloatfix}%\usepackage{stfloats}
%\usepackage[doublespacing,nodisplayskipstretch]{setspace}
%\usepackage{longtable}
%\usepackage{doi}
%\usepackage[numbers]{natbib}
%\usepackage{natbib}
%\usepackage{dblfloatfix}
\usepackage{framed}
\usepackage[font=footnotesize]{subcaption}%\usepackage{subfig}%

\usepackage{tikz}
\usetikzlibrary{calc}
\usepackage{tkz-euclide}
%\usetkzobj{all} 
\usepackage{calc}
\usepackage{tikz,pgfplots}
\pgfplotsset{compat=1.12}
\usetikzlibrary{arrows.meta,3d,matrix,positioning,decorations.markings}


\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator{\sech}{sech}
\DeclareMathOperator{\csch}{csch}
\DeclareMathOperator{\arcsec}{arcsec}
\DeclareMathOperator{\arccot}{arcCot}
\DeclareMathOperator{\arccsc}{arcCsc}
\DeclareMathOperator{\arccosh}{arcCosh}
\DeclareMathOperator{\arcsinh}{arcsinh}
\DeclareMathOperator{\arctanh}{arctanh}
\DeclareMathOperator{\arcsech}{arcsech}
\DeclareMathOperator{\arccsch}{arcCsch}
\DeclareMathOperator{\arccoth}{arcCoth} 

% Commands for this paper
\newcommand{\ntest}{n_\mathcal{T}}
\newcommand{\test}{\mathcal{T}}
\newcommand{\src}{\mathcal{S}}
\newcommand{\xtest}{x_\test}
\newcommand{\ytest}{y_\test}
\newcommand{\xsrc}{x_\src}
\newcommand{\ysrc}{y_\src}
\newcommand{\zsrc}{z_\src}
\newcommand{\real}{\mathrm{Re}}
\newcommand{\todo}[1]{{\color{red}#1}}


% Commands
\newcommand{\maxpoly}{d}
\newcommand{\nfuncpoly}{{\tilde{m}}}

\newcommand{\ngroup}{{n_g}}

\newcommand{\nfunc}{{n_\func}}
\newcommand{\nsing}{{n_\singfunc}}
\newcommand{\nmono}{{n_\monofunc}}

\newcommand{\func}{f}
\newcommand{\singfunc}{s}
\newcommand{\monofunc}{m}

\newcommand{\funcvec}{\mathbf{\func}}
\newcommand{\singfuncvec}{\mathbf{\singfunc}}
\newcommand{\monofuncvec}{\mathbf{\monofunc}}

\newcommand{\npoints}{n}
\newcommand{\polyextra}{\delta}

\newcommand{\pz}{\phantom{0}}
\newcommand{\ps}{\phantom{-}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% The following corrects an issue with older versions of pgfplots
\makeatletter
\tikzoption{canvas is xy plane at z}[]{%
  \def\tikz@plane@origin{\pgfpointxyz{0}{0}{#1}}%
  \def\tikz@plane@x{\pgfpointxyz{1}{0}{#1}}%
  \def\tikz@plane@y{\pgfpointxyz{0}{1}{#1}}%
  \tikz@canvas@is@plane
}
\makeatother

% The following creates an arbitrary plane
\makeatletter
\tikzoption{canvas is plane}[]{\@setOxy#1}
\def\@setOxy O(#1,#2,#3)x(#4,#5,#6)y(#7,#8,#9)%
  {\def\tikz@plane@origin{\pgfpointxyz{#1}{#2}{#3}}%
   \def\tikz@plane@x{\pgfpointxyz{#4}{#5}{#6}}%
   \def\tikz@plane@y{\pgfpointxyz{#7}{#8}{#9}}%
   \tikz@canvas@is@plane
  }
\makeatother 


\definecolor{orange}{rgb}{1,0.5,0}
\definecolor{green}{rgb}{0,0.5,0}
\definecolor{purple}{rgb}{0.5,0,0.5}
\newcommand{\reviewerOne}[1]{{\color{orange}{#1}}}
\newcommand{\rereading}[1]{#1}%\newcommand{\rereading}[1]{{\color{purple}{#1}}}
\newcommand{\reviewerThree}[1]{{\color{green}{#1}}}
